UniMark: Artificial Intelligence Generated Content Identification Toolkit

The rapid proliferation of Artificial Intelligence Generated Content has precipitated a crisis of trust and urgent regulatory demands. However, existing identification tools suffer from fragmentation and a lack of support for visible compliance marking. To address these gaps, we introduce the \textbf{UniMark}, an open-source, unified framework for multimodal content governance. Our system features a modular unified engine that abstracts complexities across text, image, audio, and video modalities. Crucially, we propose a novel dual-operation strategy, natively supporting both \emph{Hidden Watermarking} for copyright protection and \emph{Visible Marking} for regulatory compliance. Furthermore, we establish a standardized evaluation framework with three specialized benchmarks (Image/Video/Audio-Bench) to ensure rigorous performance assessment. This toolkit bridges the gap between advanced algorithms and engineering implementation, fostering a more transparent and secure digital ecosystem.

==> 2.System_Design.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{System Design}\label{system_design}

\subsection{Unified Engine Architecture}
The core of the \textbf{UniMark} is the \texttt{UnifiedWatermarkEngine}, designed to abstract the complexities of multimodal processing into a cohesive framework. We employ the Facade Pattern through the \texttt{WatermarkTool} class, providing developers with a simplified, high-level interface that masks the intricate details of underlying model initialization and tensor manipulations.

A key innovation in our architecture is the Dual-Operation Strategy, as illustrated in Figure \ref{fig:architecture}. Unlike traditional systems that focus solely on invisible steganography, our engine natively supports two distinct operation modes via unified \texttt{embed} and \texttt{extract} APIs:
\begin{itemize}
    \item \textbf{Hidden Watermarking} (\texttt{operation='watermark'}): Embeds imperceptible signals for copyright protection and technical tracing, utilizing deep learning-based encoders.
    \item \textbf{Visible Marking} (\texttt{operation='visible\_mark'}): Applies explicit compliance markers (e.g., visual overlays or audio prompts) to meet regulatory transparency requirements, such as those mandated by the EU AI Act \cite{eu_ai}.
\end{itemize}

\begin{figure}[h]
    \centering
    \includegraphics[width=0.95\linewidth]{figures/system_architecture.png}
    \caption{\textbf{System Architecture of UniMark.} The Unified Engine acts as a central hub, routing user inputs through a dual-operation pathway (Hidden Watermark vs. Visible Mark) across four modalities, ensuring both copyright protection and regulatory compliance.}
    \label{fig:architecture}
\end{figure}

To ensure efficiency and scalability, the system implements a Lazy Loading mechanism. Heavy resources, such as the 1.3B parameter Wan 2.1 video generation model or the AudioSeal encoder, are instantiated only upon the first request for their specific modality. Furthermore, the entire system is Config-Driven, managed by a centralized YAML configuration (\texttt{config/default\_config.yaml}), allowing researchers to dynamically switch algorithms or adjust hyperparameters without modifying the source code.

\subsection{Multimodal Algorithm Integration}
The toolkit integrates State-of-the-Art (SOTA) algorithms across four modalities through a standardized adapter interface. In this section, we primarily detail the integration of the visual modality, followed by a brief overview of the audio and text modalities.

For both image and video modalities, we unify the backend using VideoSeal \cite{videoseal}. By treating images as single-frame videos, we leverage a single pre-trained encoder to embed watermarks that are robust against both spatial editing (e.g., cropping, resizing) and temporal manipulation (e.g., frame dropping). This approach significantly reduces code redundancy and maintenance overhead while ensuring consistent performance across visual content. Furthermore, we construct an automated pipeline that seamlessly links generative models with the watermarking process; for instance, video content generated by Wan 2.1 \cite{wan} is automatically passed to the VideoSeal encoder for immediate protection.

Regarding other modalities, we integrate AudioSeal \cite{audioseal} for audio watermarking, which enables precise identification of AI-generated segments within longer streams through localized detection. For text, we employ PostMark \cite{postmark} to address the prevalence of closed-source LLMs. Unlike generation-time methods that require access to model logits, PostMark operates as a post-processing step, ensuring our toolkit remains model-agnostic and compatible with black-box APIs such as GPT-4.


\subsection{Standardized Evaluation Framework}
To address the fragmentation in evaluation standards, we provide a comprehensive benchmarking suite located in the \texttt{benchmarks/} directory. Its primary objective is to evaluate the performance of watermark algorithms across different modalities by providing standardized test datasets, diverse attack methods, and unified evaluation metrics, thereby assisting users in selecting the most suitable algorithm for their specific application scenarios.

\begin{figure}[h]
    \centering
    \includegraphics[width=0.95\linewidth]{figures/evaluation_pipeline.png}
    \caption{\textbf{Evaluation Pipeline of UniMark.} The process follows a rigorous "Attack-Detect-Score" loop: starting with a standardized Dataset, content undergoes Watermark embedding. Quality is evaluated by comparing watermarked content with the original. Subsequently, Attack simulations (e.g., noise, compression) are applied, followed by watermark Extraction. Finally, Robustness is assessed by comparing the extracted message against the original.}
    \label{fig:eval_pipeline}
\end{figure}

We offer three specialized benchmarks covering the major modalities. \textbf{Image-Bench}, built upon the W-Bench dataset, evaluates robustness against 25 types of distortions, including common operations like JPEG compression and Gaussian blurring. \textbf{Video-Bench}, based on the VideoMarkBench dataset, focuses on temporal consistency and resistance to frame-level attacks such as frame dropping and averaging. \textbf{Audio-Bench} utilizes the AudioMark dataset to assess robustness against audio-specific perturbations like noise injection, time-stretching, and MP3 compression.

The framework evaluates algorithms across two critical dimensions: Quality and Robustness. Quality metrics measure the imperceptibility of the watermark, utilizing PSNR, SSIM, and LPIPS for visual content, and SNR for audio, to ensure that the watermarking process does not degrade the user experience. Robustness metrics quantify the detectability of the watermark under various attacks, primarily using True Positive Rate (TPR) and Bit Accuracy (BA). The \texttt{BenchmarkRunner} automates the calculation of these metrics, generating standardized reports and radar charts to facilitate fair and intuitive comparisons between different algorithms.






        




==> Appendices.tex <==
\begin{appendices}


    \end{appendices}

    
    





==> preamble.tex <==


\usepackage{fullpage}

% Language setting
% Replace `english' with e.g. `spanish' to change the document language
\usepackage[english]{babel}

% Set page size and margins
% Replace `letterpaper' with `a4paper' for UK/EU standard size
\usepackage[a4paper,top=2cm,bottom=2cm,left=3cm,right=3cm,marginparwidth=1.75cm]{geometry}

\usepackage{fullpage}
\usepackage{enumerate}
\usepackage{indentfirst}
\usepackage{graphicx}
\usepackage{amsfonts}%空心G,Z
\usepackage{amsmath}%花括号公式
\usepackage{amsthm}
\usepackage{bm}%数学字体加粗
\usepackage{makecell}
\usepackage{tikz}
\usepackage{soul}%下划线
\usepackage{framed}%文字带边框
\usepackage{tabularx} %指定表格宽度 根据内容调整宽度X
\usepackage{threeparttable} %tablenotes置顶
\usepackage{subfigure}
\usepackage{enumitem}
\usepackage{multicol}
\usepackage{multirow}
\usepackage{setspace}
\usepackage{pifont}% http://ctan.org/pkg/pifont
\usepackage{tikz, pgfplots}
\usepackage{dashrule} %文档中插入虚线
\usepackage[colorlinks, anchorcolor=blue, linkcolor=blue, citecolor=blue, urlcolor=black]{hyperref} %添加超链接
\usetikzlibrary{matrix, fit, calc, matrix, patterns, backgrounds, arrows, 
	shapes, chains, fit, decorations, intersections, positioning}





%%%% Standard Packages
%%<additional latex packages if required can be included here>
% \usepackage{todonotes}  % Add this to the preamble with other packages
\usepackage{graphicx}%

\usepackage{amsmath,amssymb,amsfonts}%
\usepackage{amsthm}%
% \newcounter{funcitonality}
% \newenvironment{funcitonality}{
%   \refstepcounter{funcitonality}
%   \textbf{Functionality \thefuncitonality}\quad
% }{}
\usepackage{mathrsfs}%
\usepackage[title]{appendix}%
% \usepackage{xcolor}%
% \usepackage{textcomp}%
% \usepackage{manyfoot}%
\usepackage{booktabs}%
% \usepackage{algorithm}%
% \usepackage{algorithmicx}%
% \usepackage{algpseudocode}%
% \usepackage{listings}%
\usepackage{stmaryrd}%\llbracket 和 \rrbracket
% \usepackage{float}% 提供 [H] 浮动选项
% \restylefloat{algorithm} % 允许对 algorithm 使用 [H]
\usepackage{caption}
\usepackage{framed}
% \usepackage{ulem}

%%%%
% \renewcommand{\algorithmicrequire}{\textbf{Input:}}
% \renewcommand{\algorithmicensure}{\textbf{Output:}}
\newtheorem{lemma}{Lemma}
%%%%%=============================================================================%%%%
%%%%  Remarks: This template is provided to aid authors with the preparation
%%%%  of original research articles intended for submission to journals published 
%%%%  by Springer Nature. The guidance has been prepared in partnership with 
%%%%  production teams to conform to Springer Nature technical requirements. 
%%%%  Editorial and presentation requirements differ among journal portfolios and 
%%%%  research disciplines. You may find sections in this template are irrelevant 
%%%%  to your work and are empowered to omit any such section if allowed by the 
%%%%  journal you intend to submit to. The submission guidelines and policies 
%%%%  of the journal take precedence. A detailed User Manual is available in the 
%%%%  template package for technical guidance.
%%%%%=============================================================================%%%%

%% as per the requirement new theorem styles can be included as shown below
\theoremstyle{thmstyleone}%
\newtheorem{theorem}{Theorem}%  meant for continuous numbers
%%\newtheorem{theorem}{Theorem}[section]% meant for sectionwise numbers
%% optional argument [theorem] produces theorem numbering sequence instead of independent numbers for Proposition
\newtheorem{proposition}[theorem]{Proposition}% 
%%\newtheorem{proposition}{Proposition}% to get separate numbers for theorem and proposition etc.

\theoremstyle{thmstyletwo}%
\newtheorem{example}{Example}%
\newtheorem{remark}{Remark}%

\theoremstyle{thmstylethree}%
\newtheorem{definition}{Definition}%

\newcommand{\blue}[1]{ {\textcolor{blue}{#1}}}


